The ATLAS Readout System for LHC Runs 2 and 3

The ReadOut System (ROS) is a central part of the data acquisition (DAQ) system of the ATLAS Experiment at the CERN Large Hadron Collider (LHC). The system is responsible for receiving and buffering event data from all detector subsystems and serving these to the High Level Trigger (HLT) system via a 10 GbE network, discarding or transporting data onward once the trigger has completed its selection process. The ATLAS ROS was completely replaced during the 2013-2014 experimental shutdown in order to meet the demanding conditions expected during LHC Run 2 and Run 3 (2015-2025). The ROS consists of roughly one hundred Linux-based 2U-high rack-mounted servers equipped with PCIe I/O cards and 10 GbE interfaces. This paper documents the system requirements for LHC Runs 2 and 3 and the design choices taken to meet them. The results of performance measurements and the re-use of ROS technology for the development of data sources, test platforms for other systems, and another ATLAS DAQ system component, namely the Region of Interest Builder (RoIB), are also discussed. Finally performance results for Run 2 operations are presented before looking at the upgrade for Run 3.

==> designoverview.tex <==
\newpage
\section{Upgraded ROS: Design overview and principal elements}
\label{sec:principaldesign}

The Run~2 \& 3 ROS system is identical in role to its predecessor and shares the majority of its functional components. The design of this upgraded system sought to make use of up to date technology to eliminate many of the known bottlenecks in the old system. Principal among these changes were the management of transfers across the PCI bus (now PCIe in the new system) and exploiting the substantial performance gains made in commodity CPU performance. Interrupt technology had also developed significantly since the design of the original system and was used to further optimise the processing model. The upgraded system was implemented with 2U high server PCs with increased processing capacity and network connectivity. The ROBIN I/O cards were replaced by the newer RobinNP cards. The RobinNP implementation has improved link density (12 S-LINK inputs per card instead of 3), memory capacity (660 MB per input instead of 64 MB) and PCIe bus bandwidth capability (measured maximum of 1.6 GB/s instead of 180 MB/s, i.e. on average 125 MB/s per input instead of 60 MB/s) compared to the original ROBIN I/O card. Most ROS PCs have two cards installed, which in combination with the reduction in height of the PCs means that 12 link can be connected per unit of height instead of 3.

In the Run~1 system data transfer and delete requests (as well as other board management operations) were handled by the ROBIN's on-board PowerPC chip. To avoid the limitations of such an architecture on future improvements, whilst also removing the need to maintain another processor technology, the decision was made to move all software functionality into the process running on the host PC. This provides a simpler software interface and makes future performance upgrades easier through simply upgrading the host CPU. In order for this approach to proceed a mechanism was needed to minimise the overhead of communicating across the PCIe bus, which could otherwise eliminate most of the benefit of the new processing model.

The new system eliminated polling by making use of software threads that sleep in the case a FIFO becomes empty and are woken up by an interrupt, process all available data in the FIFO, and then sleep again. This is made possible by improvements in interrupt latency in modern architectures, meaning that the overheads don't counteract the gains. The new model, using both interrupts and features such as semaphores and inter-thread signalling, has the added benefit that it is now possible to effectively monitor the load on the system via CPU utilisation, whereas with the Run~1 system all cores were always 100\% busy due to tight polling. 

In the following sections the key functional and design elements of the ROS will be described and discussed in more detail.
